Efficient Learning of Voltage Control Strategies via Model-based Deep Reinforcement Learning

This article proposes a model-based deep reinforcement learning (DRL) method to design emergency control strategies for short-term voltage stability problems in power systems. Recent advances show promising results in model-free DRL-based methods for power systems, but model-free methods suffer from poor sample efficiency and training time, both critical for making state-of-the-art DRL algorithms practically applicable. DRL-agent learns an optimal policy via a trial-and-error method while interacting with the real-world environment. And it is desirable to minimize the direct interaction of the DRL agent with the real-world power grid due to its safety-critical nature. Additionally, state-of-the-art DRL-based policies are mostly trained using a physics-based grid simulator where dynamic simulation is computationally intensive, lowering the training efficiency. We propose a novel model-based-DRL framework where a deep neural network (DNN)-based dynamic surrogate model, instead of a real-world power-grid or physics-based simulation, is utilized with the policy learning framework, making the process faster and sample efficient. However, stabilizing model-based DRL is challenging because of the complex system dynamics of large-scale power systems. We solved these issues by incorporating imitation learning to have a warm start in policy learning, reward-shaping, and multi-step surrogate loss. Finally, we achieved 97.5% sample efficiency and 87.7% training efficiency for an application to the IEEE 300-bus test system.

==> extra.tex <==
% \IEEEPARstart{R}{ecent} studies \cite{glavic2019deep,cao2020reinforcement,huang2019adaptive} show that deep reinforcement learning (DRL) methods have made significant progress in providing fast and effective solutions compared to the traditional rule-based and optimization-based (e.g., model predictive control) methods in power system stability and emergency control applications. DRL-based control policies are predominantly trained in a simulated environment  instead of directly interacting with the real-world power grid due to high safety and security requirements of power systems. For first-principle-based dynamic modeling of large-scale power system systems, large-scale differential algebraic equation (DAE) models have to be solved, which is computationally intensive. Considering the large amount of explorations required for DRL training, this leads to extensive training and tuning time to obtain a good DRL-based control policy for large-scale power systems. In earlier work \cite{huang2021accelerated}, we developed parallel augment random search (PARS), a derivative-free DRL algorithm and reduced the DRL-based policy training time for power systems from days to hours. However, it is rather challenging to further reduce the training time given the computing resource limit, due to the use of computationally intensive grid simulators in the training loop.




% Reinforcement learning (DRL) methods can be categorized into two classes: model-free and model-based. In the model-free methods, DRL agents learn through interacting with the environment directly. Most of the existing DRL works in power systems belong to this class. Compared to model-free approaches, model-based approaches first learn a surrogate (or transition) model of the system dynamics and obtain an optimal policy through interacting with the learned surrogate model.    Compared to first-principle physics-based models, surrogate dynamic models can be much lower dimensional, thus computationally more efficient, while preserving the key dynamics of the systems. Thus, there is a good potential to reduce the training time by using a surrogate model instead of grid simulators and realizing model-based deep reinforcement learning (MB-DRL).  However, there are known challenges in achieving this due to a combination of challenges in deriving a good surrogate model for large-scale, complex power systems, modeling error accumulation and state-action distribution drifting. To the best of our knowledge, there is no systematic study of MB-DRL methods in terms of feasibility and applicability for bulk power system dynamic stability control applications.    

% In this paper, we developed a novel MB-DRL framework that significantly accelerates the training process and improves learning efficiency compared to the model-free methods.  We overcame several challenges in training DRL policy with a learned surrogate model by introducing (i) multi-step loss in model learning, (ii) regular update of surrogate models in the DRL training loop, (iii) robust reward structure, and (iv) imitation learning.  Our method resulted in a notable reduction (i.e., 8X in the IEEE 300-bus test case) of DRL training time. We believe this is a major boost in making DRL practical for real-world grid control applications.


% {\color{blue} \subsubsection{Standard Approaches on Model-based RL} A comprehensive survey on MBRL methods can be found in the recent review \cite{luo2022survey}. MBRL has mainly two components: Model learning and Model usage for Policy learning. Model learning from historical data can be achieved using (a) Tabular methods and (b) Prediction loss. Tabular settings are adopted in early research and are only effective in applications with finite state and action spaces \cite{sutton1990integrated,brafman2002r}, hence are not suitable for complex real-world systems. One-step transition model using prediction loss is utilized in many recent works \cite{kurutach2018model,nagabandi2018neural,janner2019trust}. Among them, \cite{nagabandi2018neural} learns a deterministic model with single-step prediction loss using supervised learning over the collected trajectory data. A deterministic model often fails to capture the inherent stochasticities of the environment - this requires a probabilistic model introduced in \cite{pilco,gal2016improving,buesing2018learning,chua2018deep} with uncertainty measure of the learned model. \cite{janner2019trust,xu2020error} emphasized finding a performance bound between the returns obtained in the model-based and ground truth process. To bound model error, \cite{venkatraman2015improving} introduced Lipschitz bound on learned model. Apart from one-step prediction model \cite{talvitie2017self,pmlr-v100-yang20a,asadi2019combating} utilized multi-step loss-based prediction model to make the learned model more accurate in long-horizon trajectory predictions. Besides, the model learned by distribution matching is achieved in \cite{shi2019virtual}. 

% In Model usage for Policy learning, Dyna-Q \cite{sutton2018reinforcement} proposed a planning stage before the policy learning resulting in a policy search through a trained-dynamic model. A common way to formulate policy learning with the learned dynamic model is to utilize the model predictive control (MPC) framework \cite{nagabandi2018neural,chua2018deep,pmlr-v100-yang20a}. \cite{nagabandi2018neural} utilized learned model-based random shooting with model-free fine-tuning for policy learning. To improve data efficiency and sample complexity in policy search \cite{chua2018deep,pmlr-v100-yang20a} adopted the cross entropy-based methods (CEM) over the simple random shooting method. 
% % Unlike random shooting, in CEM, the actions are selected from some non-uniform candidate distribution (for instance, the normal distribution used in \cite{pmlr-v100-yang20a}). Then, the candidate distribution is improved based on the best sample solution \cite{chua2018deep} obtained at each iteration step. 
% On the other hand, some model-based RL work used the algorithms primarily used in the model-free setting. Among them, \cite{janner2019trust} adopted soft-actor critic (SAC) \cite{haarnoja2018soft} as their algorithm of model-based policy optimization. \cite{kaiser2019model} uses proximal policy gradient (PPO) \cite{schulman2017proximal} in the policy learning with the neural network-based simulated environment for atari games. While, \cite{feinberg2018model} introduced a learned model-based value expansion method in connection to the deep deterministic policy gradient (DDPG) \cite{lillicrap2020continuous} algorithm. Here, the main intention was to replace the actual Q function of the DDPG algorithm using a model-based proxy Q-function, thereby reducing the sample complexity of learning. In another work, PILCO \cite{pilco} uses a probabilistic model, learns the policy using the bayesian approximate inference method, and later performs analytical gradient-based updates in policy improvement. Dyna-DQN \cite{holland2018effect}, a straightforward extension of Dyna-Q for application in high dimensional state and action space, incorporates the popular Deep-Q-Networks (DQN) \cite{mnih2015human} in the Dyna framework. 
% Depending on the policy learning algorithm, it should be essential to note that both random shooting and CEM are derivative-free methods. At the same time, SAC, PPO, DDPG, and PILCO belong to the policy gradient algorithms, and Dyna-Q and Dyna-DQN are value-function-based methods.


%For a given set of state-transition tuple $\mathcal{D} = \{(s_t,a_t,s_{t+1})\}$, the single step estimation error is given in (\ref{eqn_1steploss}),
% \begin{align} \label{eqn_1steploss}
%     \mathcal{L}_{ss}(\theta) = \frac{1}{\lvert\mathcal{D}\rvert} \sum_{(s_t,a_t,s_{t+1})\in \mathcal{D}} \Big \lVert {s_{t+1} - s_t - f_{\phi}(s_t,a_t)}\Big \rVert_2^2
% \end{align}
% The use of single step loss function $\mathcal{L}_{ss}(\theta)$ can produce reasonably good prediction for next state $\hat{s}_{t+1}$, but it is obvious that there should be certain mismatch between $\hat{s}_{t+1}$ and its ground truth version $s_{t+1}$, producing an error term $\varepsilon_t = \lvert s_{t+1} - s_t \rvert$. Next, when we use the trained model to propagate the dynamics for long horizon roll-outs, these error terms $\varepsilon \lvert_{t=0}^{T}$ get accumulated. Hence, with single step loss function, the trained model fails to prevent accumulation of error for long horizon prediction and would certainly makes the optimal policy learning difficult for the DRL agent. To solve this problem, we used multi-step loss function \cite{talvitie2017self,pmlr-v100-yang20a} as defined in (\ref{eqn_mult_step_loss}) while training the DNN representing $f_{\phi}(\cdot,\cdot)$. 

% Further, in recent studies, it is found that these methods \cite{mania2018simple} are highly scalable alternatives compared to the gradient-based and value-based methods. %The derivative-free methods, random shooting, and CEM mentioned earlier relies on simple candidate distribution for action search, hence they are not suitable for high dimensional search space, which is the case in power grid control problems.
% Therefore, we adopt the derivative-free PARS algorithm with DNN-based policy network in this model-based RL setting. Details of the proposed algorithm is presented in Section \ref{sec3} in connection to the power systems problem.


%\subsection{Improving Model Accuracy during Policy Learning}\label{sec2d}

% motivated by the fact that the mismatch between state-action distribution used in the training of $f_{\phi}(s_t,a_t)$ and the one currently observed by the policy $\pi(s_t)$ \cite{ross2011reduction} needs to be reduced. Here, it is important to note that the policy function $\pi(\cdot)$ changes as learning goes on. Therefore, to minimize the distribution mismatch, the ground truth trajectories are collected online using the current policy $\pi(\cdot)$ and stored as a separate data set (from the initially collected offline data), utilized in the intermediate training of $f_{\phi}(s_t,a_t)$.


%This online collected new training data set comes from the state-action distribution where the policy is currently existing. Next, the dynamic model $f_{\phi}(s_t,a_t)$ is trained at a regular interval in parallel to the policy learning with the combined set of old and new data. With this, the model accuracy improves on the parts of state-action space observed by the current policy $\pi(\cdot)$, which in turn helps in policy learning. 

% Hence, $f_{\phi}(s_t,a_t)$ works satisfactory close to the nominal trajectories, which are used for its training. 
% Using learned models for action planning raises extra challenges for model accuracy. Although a learned dynamics model can generally remain accurate around trajectories in the training data, its performance for unseen state-actions is not guaranteed. As a result, the planner might exploit such imperfections in the model and optimize for actions that are actually suboptimal on the robot. To compensate for this distribution mismatch between training and testing data, we keep track of all collected trajectories in a replay buffer and periodically retrain the model using all trajectories [18]. The updated model is then used to collect more trajectories from the robot, which are added to the replay buffer for future model training (Fig. 1). By interleaving model training and data collection, we improve the model’s accuracy on parts of the state space where the planner is more likely to visit, which in turn increases the quality of the plan.


% The most important part of any DRL-based method is to derive the optimal policy for the task under consideration. As discussed earlier, in the model-based method, this part is even more challenging as the training of the policy is done with a learned dynamic model. 
% A common way to formulate the policy learning with the learned dynamic model is to utilize the model predictive control (MPC) framework \cite{nagabandi2018neural,chua2018deep,pmlr-v100-yang20a}. By definition, MPC uses the current state information and computes a sequence of control actions optimizing the system trajectory over an admissible set of control actions. Then, it applies the immediate control action and recomputes another sequence of control action starting from the actual state measurement obtained in the next step. This periodic re-planning provides MPC the flexibility of optimizing through an inexact or approximated model. But, finding the exact optimum through MPC, using analytical optimization, is difficult considering the complexity in dynamics and reward structure. To this end, \cite{nagabandi2018neural} used a random-sampling-based shooting method in learning the optimal policy through the learned dynamics. The method deals with selecting $K$ randomly generated candidate action sequences $a^{\text{seq}}_t=\{a_t,\cdots,a_{t+H-1}\}$ (for a horizon of $H$ time-steps), then the trajectory roll-outs are generated using the dynamics given by $s_{t+1} = s_t + f_{\phi}(s_t,a_t)$ and corresponding cumulative rewards are computed for the same time period using the formula, $\sum_{t}^{t+H-1} \gamma^t r(s_t,a_t,s_{t+1})$. Now, the candidate action sequence that gives the maximum cumulative reward is chosen as the optimum one. The process is repeated for the next $H$ steps starting from $t+1$ after executing only the first action of the action sequence computed at $t$. 
